Synthetic Data Generation Techniques for Developing AI-based Speech Assessments for Parkinson's Disease (A Comparative Study)

Changes in speech and language are among the first signs of Parkinson's disease (PD). Thus, clinicians have tried to identify individuals with PD from their voices for years. Doctors can leverage AI-based speech assessments to spot PD thanks to advancements in artificial intelligence (AI). Such AI systems can be developed using machine learning classifiers that have been trained using individuals' voices. Although several studies have shown reasonable results in developing such AI systems, these systems would need more data samples to achieve promising performance. This paper explores using deep learning-based data generation techniques on the accuracy of machine learning classifiers that are the core of such systems.

==> ExplainabilityResults.tex <==

\begin{figure*}
  \begin{minipage}[t]{.3\linewidth}
    \includegraphics[width=\linewidth]{images/TAVE_Patients.png}%
    \caption{The influences of features on the classification result of test samples from the patients class. Among 17 features, the ppe and spread 1 have highest impact on the classification results.}%
  \end{minipage}\hfil
  \begin{minipage}[t]{.3\linewidth}
    \includegraphics[width=\linewidth]{images/CTGAN1.png}%
    \caption{The influences of features on the classification result of test samples from the patients class. Among  22 features, the ppe and mdvp\_shimmer\_db have highest impact on the classification results.}%
  \end{minipage}\hfil
  \begin{minipage}[t]{.3\linewidth}
    \includegraphics[width=\linewidth]{images/shap_cap.png}%
    \caption{The influences of features on the classification result of test samples from the patients class. Among  12 features, the shimmer\_apq5 and spread1 have highest impact on the classification results.}%
  \end{minipage}%
\end{figure*}


\begin{table}[t]
\centering
\caption{List of features}
\begin{tabular}{|c|c|c|c|}
\hline
 \textbf{Feature} & \textbf{TVAE}  & \textbf{CTGAN} &
 \textbf{CopulaGAN}\\
\hline
mdvp\_fo\_hz & Feature 0& Feature 0&Feature 0\\
mdvp\_fhi\_hz & &Feature 1&Feature 1\\
mdvp\_flo\_hz &Feature 1 & Feature 2& \\
mdvp\_jitter & & Feature 3& \\
mdvp\_jitter\_abs & &Feature 4 & \\
mdvp\_rap &Feature 2 & Feature 5& Feature 2\\
mdvp\_ppq & Feature 3& Feature 6& Feature 3\\
jitter\_ddp & Feature 4& Feature 7& Feature 4\\
mdvp\_shimmer &Feature 5 &Feature 8& Feature 5\\
mdvp\_shimmer\_db &Feature 6 & Feature 9& \\
shimmer\_apq3 & & Feature 10& \\
shimmer\_apq5 & Feature 7& Feature 11& Feature 6\\
mdvp\_apq & Feature 8&  Feature 12&Feature 7\\
shimmer\_dda & Feature 9& Feature 13& \\
nhr & Feature 10& Feature 14& \\
hnr & Feature 11& Feature 15& \\
rpde & Feature 12& Feature 16& Feature 8\\
dfa & & Feature 17& \\
spread1 & & Feature 18& Feature 9\\
spread2 &Feature 14 & Feature 19& Feature 10\\
d2 &Feature 15 & Feature 20& \\
ppe &Feature 16& Feature 21& Feature 11\\
\hline
\end{tabular}
\label{tab:FeaturesList}
\end{table}



==> explainability.tex <==

Finally, we applied Shapley Additive exPlanations (SHAP) \cite{lundberg2017unified} as a model-agnostic explainable model, to explain the classifiers' outputs.
